MAPS-X: Explainable Multi-Robot Motion Planning via Segmentation

Traditional multi-robot motion planning (MMP) focuses on computing trajectories for multiple robots acting in an environment, such that the robots do not collide when the trajectories are taken simultaneously. In safety-critical applications, a human supervisor may want to verify that the plan is indeed collision-free. In this work, we propose a notion of explanation for a plan of MMP, based on visualization of the plan as a short sequence of images representing time segments, where in each time segment the trajectories of the agents are disjoint, clearly illustrating the safety of the plan. We show that standard notions of optimality (e.g., makespan) may create conflict with short explanations. Thus, we propose meta-algorithms, namely multi-agent plan segmenting-X (MAPS-X) and its lazy variant, that can be plugged on existing centralized sampling-based tree planners X to produce plans with good explanations using a desirable number of images. We demonstrate the efficacy of this explanation-planning scheme and extensively evaluate the performance of MAPS-X.

==> sections/notUsed/benchmark.tex <==
% \begin{table*}[t]
%   \centering
%   \begin{tabular}{||c| c c c c c c c c c c c ||}
%     \hline
%        & Space & Planner & Dyn. & \shortstack{\# \\ of \\ Agents} & r & \shortstack{\% of \\Solutions \\ Found} & \shortstack{Computation \\ Time} & \shortstack{Computation \\Time \\ Success} & \shortstack{Average \\ Cost} & \shortstack{Segmentation \\ Time} & $\shortstack{States \\ per \\ Second}$ \\ [0.5ex] 
%     \hline\hline
%     % Crossing & MAPS-EST & $1^{st}$ Order Linear & 2 & $\infty$ & 14.5 & $28 \pm 5$ & $17 \pm 8$ & $1 \pm 1$ & $2700 \pm 52$ \\ 
%     % \hline
%     % Crossing & MAPS-RRT & $1^{st}$ Order Linear & 2 & $\infty$ & 100 & $4 \pm 3$ & $4 \pm 3$ & $1 \pm 1$ & $2100 \pm 119$ \\
%     % \hline
%     % T-Intersection & MAPS-EST & $1^{st}$ Order Linear & 2 & $\infty$ & 19.7 & $27 \pm 7$ & $8 \pm 4$ & $1 \pm 1$ & $2870 \pm 33$ \\
%     % \hline
%     %Open & MAPS-RRT & 1L & 2 & $\infty$ & 100 & $4 \pm 4$ & $4 \pm 4$ & $2 \pm 1$ & $1 \pm 1$ & $2200 \pm 133$ \\
%     % \hline
%     % Corridor & MAPS-EST & $1^{st}$ Order Unicycle & 2 & $\infty$ & 54 & $60 \pm 10$ & $20 \pm 20$ & $n/a$ & $1700 \pm 51$ \\
%     % \hline
%     % Hallway & MAPS-EST & $1^{st}$ Order Linear & 3 & $\infty$ & 85 & $150 \pm 94$ & $130 \pm 76$ & $n/a$ & $326 \pm 5$ \\
%     % \hline
%     % Hallway & MAPS-RRT & $1^{st}$ Order Linear & 3 & $\infty$ & 99.7 & $30 \pm 41$ & $30 \pm 40$ & $2 \pm 2$ & $400 \pm 18$ \\
%     \hline
%     1& Open & MAPS-RRT & 1C & 2 & $\infty$ & 100 & $4 \pm 3$ & $4 \pm 3$ & $2 \pm 1$ & $0.8 \pm 0.5$ & $1300 \pm 75$ \\
%     \hline
%     2& Open & Lazy MAPS-RRT & 1C & 2 & $\infty$ & 100 & $3 \pm 2$ & $3 \pm 2$ & $2 \pm 1$ & $0.12 \pm 0.01$ & $1600 \pm 94$ \\
%     \hline
%     3& Open & MAPS-RRT & 1C & 2 & 1 & 90.5 & $11 \pm 9$ & $9 \pm 6$ & $1 \pm 0$ & $4 \pm 3$ & $800 \pm 99$ \\
%     \hline
%     4& Open & Lazy MAPS-RRT & 1C & 2 & 1 & 7.2 & $20 \pm 11$ & $12 \pm 9$ & $1 \pm 0$ & $2 \pm 1$ & $1200 \pm 77$ \\
%     % \hline
%     % Congested & MAPS-RRT & $2^{nd}$ Order Unicycle & 2 & 1 & 18 & $90 \pm 21$ & $50 \pm 25$ & $47 \pm 10$ & $200 \pm 25$ \\
%     \hline
%     5& Congested & MAPS-RRT & 2C & 2 & 2 & 51 & $400 \pm 200$ & $200 \pm 140$ & $2 \pm 0$ & $47 \pm 10$ & $220 \pm 52$ \\
%     \hline
%     6&Congested & MAPS-RRT & 2C & 2 & 7 & 95.6 & $35 \pm 30$ & $52 \pm 20$ & $6 \pm 1$ & $10 \pm 2$ & $570 \pm 56$ \\
%     \hline
%     7&Congested & MAPS-RRT & 2C & 2 & $\infty$ & 100 & $40 \pm 41$ & $40 \pm 41$ & $7 \pm 2$ & $6 \pm 1$ & $600 \pm 60$\\
%     \hline
%     8&Corridor & MAPS-RRT & 1U & 2 & 6 & 84.3 & $30 \pm 37$ & $20 \pm 23$ & $4 \pm 1$ & $8 \pm 9$ & $600 \pm 188$ \\
%     \hline
%     9&Corridor & MAPS-RRT & 1U & 2 & $\infty$ & 88.6 & $30 \pm 33$ & $20 \pm 20$ & $5 \pm 2$ & $5 \pm 5$ & $600 \pm 172$ \\
%     \hline
%   \end{tabular}
%   \caption{Benchmark Results}
%   \label{tab:table_benchmark_unlimited}
% \end{table*}



\begin{table*}[tbh]
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabu}{|c| l l c c c c c c c c c |}
    \hline
       & Space & Planner & Dyn. & \shortstack{\#\\ Agents} & r & \shortstack{\% Solns. \\ Found} & \shortstack{Runtime \\ (s)} & \shortstack{Runtime \\ Success (s)} & \shortstack{Ave. \\ Cost} & \shortstack{Seg. \\ Time}(s) & $\shortstack{States \\ per sec.}$ \\ [0.5ex] 
    \hline\hline
    1& Open & MAPS-RRT & 1C & 2 & $\infty$ & 100 & $4 \pm 3$ & $4 \pm 3$ & $2 \pm 1$ & $0.8 \pm 0.5$ & $1300 \pm 75$ \\
    \hline
    2& Open & Lazy MAPS-RRT & 1C & 2 & $\infty$ & 100 & $3 \pm 2$ & $3 \pm 2$ & $2 \pm 1$ & $0.12 \pm 0.01$ & $1600 \pm 94$ \\
    \hline
    3& Open & MAPS-RRT & 1C & 2 & 1 & 90.5 & $11 \pm 9$ & $9 \pm 6$ & $1 \pm 0$ & $4 \pm 3$ & $800 \pm 99$ \\
    \hline
    4& Open & Lazy MAPS-RRT & 1C & 2 & 1 & 7.2 & $20 \pm 11$ & $12 \pm 9$ & $1 \pm 0$ & $2 \pm 1$ & $1200 \pm 77$ \\
    \tabucline[1pt]{-}
    5&Congested&MAPS-RRT&2C&2&$\infty$&100&$0.3\pm0.3$&$0.3\pm0.3$&$3\pm1$&$0.09\pm0.08$& $2100\pm152$ \\
    \hline
    6&Congested&MAPS-RRT&2C&2&3&100&$0.4\pm0.4$&$0.4\pm0.4$&$2\pm1$&$0.1\pm0.1$& $2000\pm182$ \\
    \hline
    7&Congested&MAPS-RRT&2C&2&1&100&$1\pm1$&$1\pm1$&$1\pm0$&$0.3\pm0.4$& $1400\pm262$ \\
    \hline
    8&Corridor&MAPS-RRT&1U&2&$\infty$&100&$0.5\pm0.6$&$0.5\pm0.6$&$3\pm1$&$0.1\pm0.1$& $1600\pm120$ \\
    \hline
    9&Corridor&MAPS-RRT&1U&2&4&100&$0.5\pm0.5$&$0.5\pm0.5$&$3\pm1$&$0.1\pm0.1$& $1600\pm110$ \\
    \hline
    10&Corridor&MAPS-RRT&1U&2&2&100&$0.8\pm0.8$&$0.8\pm0.8$&$2\pm0$&$0.2\pm0.3$& $1400\pm187$ \\
    \hline
    11&Corridor&MAPS-RRT&1U&2&1&100&$2\pm2$&$2\pm2$&$1\pm0$&$0.6\pm0.7$& $1000\pm182$ \\
    \hline
    12&Hallway&MAPS-RRT&2L&3&$\infty$&100&$4\pm4$&$4\pm4$&$3\pm1$&$1.1\pm0.9$& $1000\pm123$ \\
    \hline
    13&Hallway&MAPS-RRT&2L&3&3&100&$4\pm5$&$4\pm5$&$3\pm0$&$1\pm1$& $900\pm154$ \\
    \hline
    14&Hallway&MAPS-RRT&2L&3&2&IN PROGRESS&$0\pm0$&$0\pm0$&$0\pm0$&$0\pm0$& $0\pm0$ \\
    \hline
    15&Hallway&MAPS-RRT&2L&3&1&IN PROGRESS&$0\pm0$&$0\pm0$&$0\pm0$&$0\pm0$& $0\pm0$ \\
    \hline
  \end{tabu}}
  \caption{Benchmark Results}
  \label{tab:table_benchmark_unlimited}
  \vspace{-4mm}
\end{table*}














==> sections/notUsed/experiments.tex <==
% experiments

In this section, we the demonstrate the efficacy of our explanation scheme and evaluate the performance of the proposed meta-algorithms lazy MAPS-\plannerX and MAPS-\plannerX.
% experimental results of MAPS-$\plannerX$ and its Lazy variant. 
% We first introduce these frameworks in the lens of two sub-optimal motion planners: \textit{Rapidly-Exploring Random Tree (RRT)} \cite{Lavalle98rapidly-exploringrandom} and \textit{Expansive Space Tree (EST)} \cite{hsu1997path}. 
% We first illustrate the framework in the lens of two classical motion planners RRT \cite{Lavalle98rapidly-exploringrandom} and EST \cite{hsu1997path} in various environments and dynamics. 
We implemented these algorithms with two classical motion planners RRT \cite{Lavalle98rapidly-exploringrandom} and EST \cite{hsu1997path}. 
% Then, we show how MAPS-$\plannerX$ compares to Lazy MAPS-$\plannerX$ in performance.
% Finally, we show how our framework extends to optimal, and near-optimal sampling-based tree planners, which optimize over different objectives such as path length, or explainability. 
All of (MAPS-X) planners were developed using the \textit{Open Motion Planning Library} (OMPL) \cite{sucan2012the-open-motion-planning-library} and are available here
% \href{https://github.com/JustinKottinger/MAPS-X}{github.com/JustinKottinger/MAPS-X}. 
\cite{mapsx-code}.
The benchmarks were performed on a machine with AMD Ryzen 7 3.9 GHz CUP and 64 GB of RAM.

% The evaluations were preformed in 5 environments with various levels of difficulty.  We also varied the dynamics and number of agents.

% \subsection{Dynamics}
% \label{sec:dynamics}
% We in these case studies, we use the following dynamics:

\subsection{MAPS Planning}
% \subsubsection{MAPS-RRT}

% \begin{figure}[htb]
% \centering
% \includegraphics[width=0.45\linewidth]{figures/mapsRRT/2ndOrderCar/example1/fullPlan.png}
% \caption{Solution via RRT in an open space}
% \label{example1_fullPlan_2ndOrderCar}
% \end{figure}

We begin with a simple proof of concept. Fig.~\ref{example1_fullPlan_2ndOrderCar} shows an example solution of the continuous \mmp problem produced by RRT. The example shows two agents, each with $2^\text{nd}$ order car dynamics that cross each others' paths to get to their goals.
% \begin{align}
% \x{i} & = \begin{bmatrix}
% x\\
% y\\
% v\\
% \phi\\
% \theta\\
% \end{bmatrix}, &  \xDot{i}&=\begin{bmatrix}
% v \cos(\theta)\\
% v \sin(\theta)\\
% a\\
% \dot{\phi}\\
% \frac{v}{L} \tan{\phi}\\
% \end{bmatrix},          &  \cntrl{i}& \begin{bmatrix}
% a\\
% \dot{\phi}\\
% \end{bmatrix}
% \label{2ndOrderCar}
% \end{align}
% It would be difficult for a human user to validate that this plan is collision free since the trajectories of the agents intersect. 
It would be difficult for a human user to validate that this plan is safe (collision free).
 % since the trajectories of the agents intersect.
The validation process becomes intuitive with MAPS-RRT 
because it is clear how the individual agents evolve in the workspace over time as shown in Figs.~\ref{fig:ex1seg1}-\ref{fig:ex1seg2}. 
In this environment, it is difficult to get smaller number of explanations.
% The explanation scheme is shown in 
% Fig.~\ref{fig:explanationEx1}.
Figs.~\ref{fig:ex1seg1}-\ref{fig:ex1seg2}.

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderCar/example1/fullPlan.png}
        \caption{Full Solutions}
        \label{example1_fullPlan_2ndOrderCar}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mapsRRT/2ndOrderCar/example1/seg1.png}
         \caption{$\dt_1 = [0, 38.5]$s}
         \label{fig:ex1seg1}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mapsRRT/2ndOrderCar/example1/seg2.png}
         \caption{$\dt_2 = [38.5, 45.5]$}
         \label{fig:ex1seg2}
     \end{subfigure}
     \caption{Open Space 1: solutions via RRT and MAPS-RRT.}
     \label{fig:explanationEx1}
\end{figure}
Instead in environment in Fig.\ref{fig:ex2Unicylce}

% \begin{figure}[htb]
% \centering
% \includegraphics[width=0.75\linewidth]{figures/mapsRRT/2ndOrderLinear/example4/fullPlan_crop.png}
% \caption{Solution via RRT in a congested space}
% \label{ex4_2ndOrderLinear}
% \end{figure}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.75\linewidth}
        \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderLinear/example4/fullPlan_crop.png}
        \caption{Solution via RRT}
        \label{ex4_2ndOrderLinear}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.75\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderLinear/example4/seg1_crop.png}
         \caption{$\dt_1 = [0, 11.7]$s}
         \label{fig:ex4Seg1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.75\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderLinear/example4/seg2_crop.png}
         \caption{$\dt_2 = [11.7, 20.2]$s}
         \label{fig:ex4Seg2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.75\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderLinear/example4/seg3_crop.png}
         \caption{$\dt_3 = [20.2, 36.9]$s}
         \label{fig:ex4Seg3}
     \end{subfigure}
        \caption{Congested space: solutions via RRT and MAPS-RRT.}
        \label{fig:ex4Linear}
\end{figure}

% \begin{align}
% \x{i} & = \begin{bmatrix}
% x\\
% y\\
% v_x\\
% v_y\\
% \end{bmatrix}, &  \xDot{i}&=\begin{bmatrix}
% v_x\\
% v_y\\
% a_x\\
% a_y\\
% \end{bmatrix},          &  \cntrl{i}& \begin{bmatrix}
% a_x\\
% a_y\\
% \end{bmatrix}
% \label{2ndOrderLinear}
% \end{align}
The need for an explanation scheme is more obvious in more complex scenarios. Consider the solution shown in Fig~\ref{ex4_2ndOrderLinear}. This example creates a double-helix-like behavior between agents that follow $2^{nd}$ order linear dynamics. 
% outlined in Eqn.~\ref{2ndOrderLinear}. 
We know that our correct algorithm generated a correct solution. However, 
the validity of the plan may be called into question when presented to a non-expert human user. The explanation scheme generated by MAPS-RRT easily avoids this problem by presenting the plan to the human in disjoint segments. 
% Fig.~\ref{fig:ex4Linear} 
Figs.~\ref{fig:ex4Seg1}-\ref{fig:ex4Seg3} 
makes it clear that the blue agent travels through the narrow corridor first, and the red agent follows, avoiding collision entirely.

% \begin{figure}[htb]
% \centering
% \includegraphics[width=0.45\linewidth]{figures/mapsRRT/2ndOrderLinear/3AgentsExample2/fullPlan_crop.png}
% \caption{Solution via RRT with 3 agents}
% \label{3agents_2ndOrderLinear}
% \end{figure}

\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.18\linewidth}
        \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderLinear/3AgentsExample2/fullPlan_crop.png}
        \caption{Full solution}
        \label{3agents_2ndOrderLinear}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderLinear/3AgentsExample2/seg1_crop.png}
         \caption{$\dt_1 = [0, 17.1]$s}
         \label{fig:3agentsSeg1}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderLinear/3AgentsExample2/seg2_crop.png}
         \caption{$\dt_2 = [17.1, 34.6]$s}
         \label{fig:3agentsSeg2}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderLinear/3AgentsExample2/seg3_crop.png}
         \caption{$\dt_3 = [34.6, 38.1]$s}
         \label{fig:3agentsSeg3}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderLinear/3AgentsExample2/seg4_crop.png}
         \caption{$\dt_4 = [38.1, 58.2]$s}
         \label{fig:3agentsSeg}
     \end{subfigure}
        \caption{Solution via RRT and MAPS-RRT with 3 agents}
        \label{fig:3agents_explained_Linear}
\end{figure*}

Validating trajectories without explanations only gets more difficult as the number of agents increase. For example, consider the solution shown in Fig.~\ref{3agents_2ndOrderLinear} where the agents 
have $2^{nd}$ order linear dynamics.
% are modeled by Eqn.~\ref{2ndOrderLinear}. 
A human user could have a difficult time checking that the entire trajectory is collision free. However, planning with the MAPS framework presents an easily verified solution, as shown in Fig.~\ref{fig:3agents_explained_Linear}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{MAPS-EST}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsEST/2ndOrderUnicycle/seg1_crop.png}
         \caption{$\dt_1 = [0, 22.1] s$}
         \label{fig:ex2Seg1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsEST/2ndOrderUnicycle/seg2_crop.png}
         \caption{$\dt_2 =[22.1, 48.9] s$}
         \label{fig:ex2Seg2}
     \end{subfigure}
     \caption{Solution via MAPS-EST in a test environment.}
     \label{fig:ex2Unicylce}
\end{figure}

We now present results of a MAPS-EST plan to show the versatility of our framework. In the example shown in Fig.~\ref{fig:ex2Unicylce}, we consider two agents governed by the $2^{nd}$ order unicycle dynamics.
% shown Equation~\ref{2ndOrderUnicycle}. 
% \begin{align}
% \x{i} & = \begin{bmatrix}
% x\\
% y\\
% v\\
% \theta \\
% \omega \\
% \end{bmatrix}, &  \xDot{i}&=\begin{bmatrix}
% v \cos(\theta)\\
% v \sin(\theta)\\
% a\\
% \omega \\
% \alpha \\
% \end{bmatrix},          &  \cntrl{i}& \begin{bmatrix}
% a\\
% \alpha\\
% \end{bmatrix}
% \label{2ndOrderUnicycle}
% \end{align}
\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{figures/mapsEST/2ndOrderUnicycle/fullPlanOneSeg_crop.png}
    \caption{MAPS-EST returns the optimal explanation scheme.}
    \label{fig:ex2_OneSegment}
\end{figure}
Now we address how the user-defined segment bound $r$ affects system behavior. 
% Consider the space in Fig.~\ref{fig:ex2Unicylce}. 
Environment in Fig.~\ref{fig:ex2Unicylce} allows a plan to be explained in one segment if the blue agent were to go around the red agent, however it is easiest for both agents to travel straight to goal. The MAPS framework enables the user to determine which behavior they would prefer. If the user would prefer an intuitive motion plan, but a suboptimal explanation scheme, they could set $r$ to be unlimited and Fig.~\ref{fig:ex2Unicylce} could be the result. Alternatively, the user could change the behavior of the system by limiting the cost bound $r$ to a single segment. An example of this behavior is shown in Fig.~\ref{fig:ex2_OneSegment}. An optimal explanation scheme would be essential in a time-critical situation where trajectory validation would need to occur as fast as possible.  



\subsection{MAPS-$\plannerX$ vs Lazy MAPS-$\plannerX$}
We now present benchmark results to show how Lazy MAPS-$\plannerX$ and MAPS-$\plannerX$
compare against differing objectives. To demonstrate, we will use the open space depicted in Fig.~\ref{fig:ex2Unicylce}, \ref{fig:ex2_OneSegment} and \ref{fig:ex2_OneSegmentSST} with the $1^{st}$ order car.
 % dynamics shown in Eqn.~\ref{1stOrderCar}. 
The space allows us to see how the planners operate for two objectives: generating a more intuitive trajectory, or an optimal explanation scheme. Each planner was run 1000 times with RRT for a maximum of 30 seconds.

\begin{figure}[htb]
\centering
\includegraphics[width=0.45\linewidth]{figures/mapsEST/2ndOrderCar/example3/fullPlan_crop.png}
\caption{Solution via EST in a narrow alley}
\label{fig:ex3_2ndCar}
\end{figure}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsEST/2ndOrderCar/example3/seg1_crop.png}
         \caption{Time Period $[0, 24.5] s$}
         \label{fig:ex3Seg1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsEST/2ndOrderCar/example3/seg2_crop.png}
         \caption{Time Period $[24.5, 41.2] s$}
         \label{fig:ex3Seg2}
     \end{subfigure}
     \caption{Solution via MAPS-EST in a narrow alley.}
     \label{fig:ex3_2ndCar_explained}
\end{figure}


\jk{need to decided if/where Fig.~\ref{fig:ex3_2ndCar}, and Fig.~\ref{fig:ex3_2ndCar_explained} fit into this section. Eqn.~\ref{2ndOrderCar} with MAPS-EST}

% \begin{align}
% \x{i} & = \begin{bmatrix}
% x\\
% y\\
% \theta \\
% \end{bmatrix}, &  \xDot{i}&=\begin{bmatrix}
% v \cos(\theta)\\
% v \sin(\theta)\\
% \frac{v}{L} \tan{\phi}\\
% \end{bmatrix},          &  \cntrl{i}& \begin{bmatrix}
% v\\
% \phi\\
% \end{bmatrix}
% \label{1stOrderCar}
% \end{align}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.75\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/benchmark/unlimited/comp_time_success.png}
         \caption{Total Computation Time}
         \label{fig:compTime_unlimited}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.75\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/benchmark/unlimited/seg_times.png}
         \caption{Time spent segmentating nodes}
         \label{fig:seg_time_unlimited}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.75\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/benchmark/unlimited/avg_states_p_sec.png}
         \caption{Average States per Second per Run}
         \label{fig:states_per_second_unlimited}
     \end{subfigure}
     \hfill
     % \begin{subfigure}[b]{0.75\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth]{figures/benchmark/unlimited/num_sols.png}
     %     \caption{Number of Solutions Found}
     %     \label{fig:sols_unlimited}
     % \end{subfigure}
     \caption{Lazy MAPS-RRT vs. MAPS-RRT: no $r$ bound.}
     \label{fig:bench_unlimited}
\end{figure}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.75\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/benchmark/limited/comp_time_success.png}
         \caption{Total Computation Time}
         \label{fig:compTime_limited}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.75\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/benchmark/limited/seg_times.png}
         \caption{Time spent segmentating nodes}
         \label{fig:seg_time_limited}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.75\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/benchmark/limited/avg_states_p_sec.png}
         \caption{Average States per Second per Run}
         \label{fig:states_per_second_limited}
     \end{subfigure}
     \hfill
     % \begin{subfigure}[b]{0.75\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth]{figures/benchmark/limited/num_sols.png}
     %     \caption{Number of Solutions Found}
     %     \label{fig:sols_limited}
     % \end{subfigure}
     \caption{Lazy MAPS-RRT vs. MAPS-RRT: $r=1$ bound.}
     \label{fig:bench_limited}
\end{figure}

The first benchmark asks how each planner performs when we do not bound $r$. Both planners found a solution on all $1000$ runs. The results are depicted in Fig.~\ref{fig:bench_unlimited}. This scenario makes planning the top priority while explainability of the solution is a second priority. Thus, Lazy MAPS-RRT benefits from finding a solution, and then segmenting it only once. This results in Lazy MAPS-RRT planning slightly faster, generate more states per second, while also spending less time calculating segmentations. It is clear that Lazy MAPS-$\plannerX$ is more desirable than MAPS-$\plannerX$ when explainability is not the first priority. 

The second benchmark asks how each planner performs when the system needs to plan for explainability. We planned in the same space as the first benchmark, for the same amount of time, with the same planning time, and the same number of runs. However, this benchmark limited the explanation scheme to a single-segment. MAPS-RRT found $905$ solutions while Lazy MAPS-RRT only found $72$. The results are shown Figure~\ref{fig:bench_limited}. It is clear that since Lazy MAPS-$\plannerX$ only segments possible solutions, the graph $G$ fails to grow in directions with satisfiable explanations, making it extremely difficult for Lazy MAPS-$\plannerX$ to generate solutions when the optimal explanation scheme conflicts with intuitive trajectories. This scenario calls for the complete MAPS-$\plannerX$ framework, as it is capable of matching desirable system behavior with an optimal explanation scheme.  

% \begin{center}
%  \begin{tabular}{||c | c c c||} 
 
% \end{tabular}
% \end{center}

% \begin{table*}[t]
%   \centering
%   \begin{tabular}{|| c | c c c c ||}
%     \hline
%         & Solutions Found & Total Computation Time Successful Trials & Segmentation Times & Average States per Second\\ [0.5ex] 
%     \hline
%     Lazy MAPS-RRT & $1000$ & $3 \pm 2$ & $0.12 \pm 0.09$ & $1625 \pm 94$ \\ 
%     \hline
%     MAPS-RRT & $1000$ & $4 \pm 3$ & $0.8 \pm 0.5$ & $1317 \pm 75$ \\
%     \hline
%   \end{tabular}
%   \caption{Benchmark Results with no $r$ bound}
%   \label{tab:table_benchmark_unlimited}
% \end{table*}

% \begin{table*}[t]
%   \centering
%   \begin{tabular}{|| c | c c c c ||}
%     \hline
%         & Solutions Found & Total Computation Time Successful Trials & Segmentation Times & Average States per Second\\ [0.5ex] 
%     \hline
%     Lazy MAPS-RRT & $72$ & $12 \pm 9$ & $2 \pm 1$ & $1156 \pm 77$ \\ 
%     \hline
%     MAPS-RRT & $905$ & $9 \pm 6$ & $4 \pm 3$ & $887 \pm 99$ \\
%     \hline
%   \end{tabular}
%   \caption{Benchmark Results with $r=1$ bound}
%   \label{tab:table_benchmark_limited}
% \end{table*}


\begin{table*}[t]
  \centering
  \begin{tabular}{|| c c c c c c c c c c ||}
    \hline
        Space & Planner & Dynamics & \shortstack{\# \\ of Agents} & r & \shortstack{\% of \\Solutions Found} & \shortstack{Computation \\ Time} & \shortstack{Computation \\Time Success} & \shortstack{Segmentation \\ Time} & $\shortstack{States \\ Second}$ \\ [0.5ex] 
    \hline\hline
    Crossing & MAPS-EST & $1^{st}$ Order Linear & 2 & $\infty$ & 14.5 & $28 \pm 5$ & $17 \pm 8$ & $1 \pm 1$ & $2700 \pm 52$ \\ 
    \hline
    Crossing & MAPS-RRT & $1^{st}$ Order Linear & 2 & $\infty$ & 100 & $4 \pm 3$ & $4 \pm 3$ & $1 \pm 1$ & $2100 \pm 119$ \\
    \hline
    T-Intersection & MAPS-EST & $1^{st}$ Order Linear & 2 & $\infty$ & 19.7 & $27 \pm 7$ & $8 \pm 4$ & $1 \pm 1$ & $2870 \pm 33$ \\
    \hline
    T-Intersection & MAPS-RRT & $1^{st}$ Order Linear & 2 & $\infty$ & 100 & $4 \pm 4$ & $4 \pm 4$ & $1 \pm 1$ & $2200 \pm 133$ \\
    \hline
    T-Intersection & MAPS-RRT & $1^{st}$ Order Car & 2 & $\infty$ & 100 & $4 \pm 3$ & $4 \pm 3$ & $0.8 \pm 0.5$ & $1300 \pm 75$ \\
    \hline
  \end{tabular}
  \caption{Benchmark Results}
  \label{tab:table_benchmark_unlimited}
\end{table*}

\input{sections/benchmark}

\subsection{Optimal MAPS Planning}
We also present examples on how our framework can be used to optimize over different objectives. First, we show MAPS-\textit{Stable Sparse RRT (SST)} \cite{li2016asymptotically}. SST is an asymptotically near-optimal motion planner for systems with kinodynamical constraints. Our MAPS variant of SST inherits these properties with the added capability of returning a satisfiable explanation scheme. Next, we append MAPS-SST to an existing meta-algorithm known as \textit{Asymptotically Optimal-$\plannerX$ (AO-$\plannerX$)} \cite{7588078}. AO-$\plannerX$ allows motion planning algorithms to optimize over any cost function by planning in the compound state-cost space. Since the cost function of MAPS-$\plannerX$ lives in $\mathbb{N}$, AO-MAPS-$\plannerX$ can be used to optimize over the number of segmentations required to explain the solution. 
\subsubsection{MAPS-SST}
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsSST/example1_2ndOrderKin/seg1_crop.png}
         \caption{Time Period $[0, 20.3] s$}
         \label{fig:ex1Seg1SST}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsSST/example1_2ndOrderKin/seg2_crop.png}
         \caption{Time Period $[20.3, 36.1] s$}
         \label{fig:ex1Seg2SST}
     \end{subfigure}
     \caption{Solution via MAPS-SST in open space.}
     \label{fig:ex1CarSST}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{figures/mapsSST/example2_2ndOrderUnicycle/fullPlanOneSeg_crop.png}
    \caption{MAPS-SST returns the optimal explanation scheme.}
    \label{fig:ex2_OneSegmentSST}
\end{figure}

Fig.~\ref{fig:ex1CarSST} shows the explanation scheme returned by MAPS-SST. Notice how the agents are more efficient in traveling to goal than in Fig.~\ref{fig:explanationEx1}. MAPS-SST can return near-optimal trajectories with satisfiable explanation schemes. If the user desired the plan to be explained in a single segment, MAPS-SST uses our cost function to return a near-optimal trajectory with an optimal explanation scheme. Fig.~\ref{fig:ex2_OneSegment} was a solution found by MAPS-SST while Fig.~\ref{fig:ex2_OneSegment} was a solution found by MAPS-EST. Despite both queries following the same dynamical constraints, the trajectories in Fig.~\ref{fig:ex2_OneSegment} more directly approach their goal region. 
\subsubsection{AO-MAPS-SST}
\jk{having some implementation issues with saving the plans for this planner. Working on fixing them now.}

==> sections/notUsed/experiments2.tex <==
% experiments

In this section, we demonstrate the efficacy of our explanation scheme and evaluate the performance of the proposed meta-algorithms Lazy MAPS-\plannerX and MAPS-\plannerX.
We implemented these algorithms with two classical motion planners RRT \cite{Lavalle98rapidly-exploringrandom} and EST \cite{hsu1997path}, 
and evaluated their performance in several environments, numbers of agents, and dynamics.  The benchmarking results are shown in Table~\ref{tab:table_benchmark_unlimited}.  See the full version of the paper \cite{Kottinger:ICRA:2020} for a more extensive analysis and evaluation.


All of %(MAPS-X) 
our
planners were developed using the \textit{Open Motion Planning Library} (OMPL) \cite{sucan2012the-open-motion-planning-library} and are available here
% \href{https://github.com/JustinKottinger/MAPS-X}{github.com/JustinKottinger/MAPS-X}. 
\cite{mapsx-code}.
The benchmarks were performed on a machine with AMD Ryzen 7 3.9 GHz CUP and 64 GB of RAM.



\subsection{MAPS Planning}

We begin with a simple proof of concept. Fig.~\ref{example1_fullPlan_2ndOrderCar} shows an example solution of the continuous \mmp problem produced by RRT. The example shows two agents, each with $2^\text{nd}$ order car dynamics that cross each others' paths to get to their goals.
It would be difficult for a human user to validate that this plan is safe (collision free).
The validation process becomes intuitive with MAPS-RRT 
because it is clear how the individual agents evolve in the workspace over time as shown in Figs.~\ref{fig:ex1seg1}-\ref{fig:ex1seg2}. 
Note that, in this environment, it is impossible to get smaller number of segments.  
\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderCar/example1/fullPlan.png}
        \caption{Full Solutions}
        \label{example1_fullPlan_2ndOrderCar}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mapsRRT/2ndOrderCar/example1/seg1.png}
         \caption{$\dt_1 = [0, 38.5]$}
         \label{fig:ex1seg1}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mapsRRT/2ndOrderCar/example1/seg2.png}
         \caption{$\dt_2 = [38.5, 45.5]$}
         \label{fig:ex1seg2}
     \end{subfigure}
     \caption{Open Space 1: solutions via RRT and MAPS-RRT.}
     \label{fig:explanationEx1}
\end{figure}

In contrast, the environment in Fig. \ref{fig:ex2Unicylce} can easily admit non-intersecting paths as the blue agent can go around the red agent (Fig. \ref{fig:ex2_OneSegment}).  However, with RRT, we often get intersecting paths 
% if we do not limit the number of explanations 
as shown in Fig. \ref{fig:ex2Seg1}-\ref{fig:ex2Seg2}.  By using MAPS-RRT and setting $r = 1$, we quickly get the easily-explainable solution in Fig. \ref{fig:ex2_OneSegment} with only one segment.
\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsEST/2ndOrderUnicycle/seg1_crop.png}
         \caption{$\dt_1 = [0, 22.1]$}
         \label{fig:ex2Seg1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsEST/2ndOrderUnicycle/seg2_crop.png}
         \caption{$\dt_2 =[22.1, 48.9]$}
         \label{fig:ex2Seg2}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/mapsEST/2ndOrderUnicycle/fullPlanOneSeg_crop.png}
        % \caption{MAPS-RRT returns the optimal explanation scheme.}
        \caption{MAPS-X $r=1$.}
        \label{fig:ex2_OneSegment}
    \end{subfigure}
     \caption{Solution via RRT and MAPS-RRT with $r=1$.}
     \label{fig:ex2Unicylce}
\end{figure}


The need for an explanation scheme is more obvious in the complex scenario in Fig. \ref{fig:ex4Linear}. Consider the solution shown in Fig~\ref{ex4_2ndOrderLinear}. This example creates a double-helix-like behavior between agents that follow $2^{nd}$ order linear dynamics, 
making it difficult for human interpretation.
The explanation scheme generated by MAPS-RRT easily explains this plan in disjoint segments in 
Figs.~\ref{fig:ex4Seg1}-\ref{fig:ex4Seg3}, 
clearly show that the blue agent travels through the narrow corridor first and the red agent follows, avoiding collision entirely.
\ml{can we get solutions with $r<3$?}
\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderLinear/example4/fullPlan_crop.png}
        \caption{Solution via RRT}
        \label{ex4_2ndOrderLinear}
     \end{subfigure}
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderLinear/example4/seg1_crop.png}
         \caption{$\dt_1 = [0, 11.7]$s}
         \label{fig:ex4Seg1}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderLinear/example4/seg2_crop.png}
         \caption{$\dt_2 = [11.7, 20.2]$s}
         \label{fig:ex4Seg2}
     \end{subfigure}
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderLinear/example4/seg3_crop.png}
         \caption{$\dt_3 = [20.2, 36.9]$s}
         \label{fig:ex4Seg3}
     \end{subfigure}
        \caption{Congested space: solutions via RRT and MAPS-RRT.}
        \label{fig:ex4Linear}
\end{figure}


Similarly, we can get better plans in terms of explanations with MAPS-X and small $r$ in the environment shown in Fig. \ref{fig:ex3Seg2}.  \ml{can we get ave number of solutions here?}


\begin{figure}[htb]
     \centering
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsEST/2ndOrderCar/example3/fullPlan_crop.png}
        \caption{Full solution}
        \label{fig:ex3_2ndCar}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsEST/2ndOrderCar/example3/seg1_crop.png}
         \caption{$[0, 24.5]$s}
         \label{fig:ex3Seg1}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsEST/2ndOrderCar/example3/seg2_crop.png}
         \caption{$[24.5, 41.2]$s}
         \label{fig:ex3Seg2}
     \end{subfigure}
     \caption{Solution via MAPS-EST in a narrow alley.}
     \label{fig:ex3_2ndCar_explained}
\end{figure}



Validating trajectories without explanations only gets more difficult as the number of agents increases. For example, consider the solution shown in Fig.~\ref{3agents_2ndOrderLinear} where the agents 
have $2^{nd}$ order linear dynamics.
A human user could have a difficult time checking that the entire trajectory is collision free. However, planning with the MAPS framework presents an easily verified solution, as shown in Fig.~\ref{fig:3agents_explained_Linear}.  By decreasing bound $r$, we can even get better explanations, e.g., the solution in Fig \ref{fig:explain-graph} was obtained with $r=3$. 
\ml{can we get solutions with $r<3$?}


\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.18\linewidth}
        \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderLinear/3AgentsExample2/fullPlan_crop.png}
        \caption{Full solution}
        \label{3agents_2ndOrderLinear}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderLinear/3AgentsExample2/seg1_crop.png}
         \caption{$\dt_1 = [0, 17.1]$s}
         \label{fig:3agentsSeg1}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderLinear/3AgentsExample2/seg2_crop.png}
         \caption{$\dt_2 = [17.1, 34.6]$s}
         \label{fig:3agentsSeg2}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderLinear/3AgentsExample2/seg3_crop.png}
         \caption{$\dt_3 = [34.6, 38.1]$s}
         \label{fig:3agentsSeg3}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsRRT/2ndOrderLinear/3AgentsExample2/seg4_crop.png}
         \caption{$\dt_4 = [38.1, 58.2]$s}
         \label{fig:3agentsSeg}
     \end{subfigure}
        \caption{Solution via RRT and MAPS-RRT with 3 agents}
        \label{fig:3agents_explained_Linear}
\end{figure*}










%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{MAPS-EST}

% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.32\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figures/mapsEST/2ndOrderUnicycle/seg1_crop.png}
%          \caption{$\dt_1 = [0, 22.1] s$}
%          \label{fig:ex2Seg1}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.32\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figures/mapsEST/2ndOrderUnicycle/seg2_crop.png}
%          \caption{$\dt_2 =[22.1, 48.9] s$}
%          \label{fig:ex2Seg2}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.32\linewidth}
%         \centering
%         \includegraphics[width=0.45\linewidth]{figures/mapsEST/2ndOrderUnicycle/fullPlanOneSeg_crop.png}
%         \caption{MAPS-RRT returns the optimal explanation scheme.}
%         \label{fig:ex2_OneSegment}
% \end{figure}
%      \caption{Solution via MAPS-EST in a test environment.}
%      \label{fig:ex2Unicylce}
% \end{figure}

% We now present results of a MAPS-EST plan to show the versatility of our framework. In the example shown in Fig.~\ref{fig:ex2Unicylce}, we consider two agents governed by the $2^{nd}$ order unicycle dynamics.
% shown Equation~\ref{2ndOrderUnicycle}. 
% \begin{align}
% \x{i} & = \begin{bmatrix}
% x\\
% y\\
% v\\
% \theta \\
% \omega \\
% \end{bmatrix}, &  \xDot{i}&=\begin{bmatrix}
% v \cos(\theta)\\
% v \sin(\theta)\\
% a\\
% \omega \\
% \alpha \\
% \end{bmatrix},          &  \cntrl{i}& \begin{bmatrix}
% a\\
% \alpha\\
% \end{bmatrix}
% \label{2ndOrderUnicycle}
% \end{align}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\linewidth]{figures/mapsEST/2ndOrderUnicycle/fullPlanOneSeg_crop.png}
%     \caption{MAPS-EST returns the optimal explanation scheme.}
%     \label{fig:ex2_OneSegment}
% \end{figure}



\subsection{MAPS-$\plannerX$ vs Lazy MAPS-$\plannerX$}

\ml{\\
- edited up to here\\
- need a discussion on the benchmarking results here and when Lazy MAPS-X performs better/worse that MAPS-X.\\
- I think we can remove the rest of the discussions below.
}


We now present benchmark results to show how Lazy MAPS-$\plannerX$ and MAPS-$\plannerX$
compare against differing objectives. To demonstrate, we will use the open space depicted in Fig.~\ref{fig:ex2Unicylce}, \ref{fig:ex2_OneSegment} and \ref{fig:ex2_OneSegmentSST} with $1^{st}$-order car dynamics.
 % dynamics shown in Eqn.~\ref{1stOrderCar}. 
The space allows us to see how the planners operate for two objectives: generating a more intuitive trajectory, or an optimal explanation scheme. Each planner was run 1000 times with RRT for a maximum of 30 seconds.




\input{sections/benchmark}


% \begin{align}
% \x{i} & = \begin{bmatrix}
% x\\
% y\\
% \theta \\
% \end{bmatrix}, &  \xDot{i}&=\begin{bmatrix}
% v \cos(\theta)\\
% v \sin(\theta)\\
% \frac{v}{L} \tan{\phi}\\
% \end{bmatrix},          &  \cntrl{i}& \begin{bmatrix}
% v\\
% \phi\\
% \end{bmatrix}
% \label{1stOrderCar}
% \end{align}

% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.75\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figures/benchmark/unlimited/comp_time_success.png}
%          \caption{Total Computation Time}
%          \label{fig:compTime_unlimited}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.75\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figures/benchmark/unlimited/seg_times.png}
%          \caption{Time spent segmentating nodes}
%          \label{fig:seg_time_unlimited}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.75\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figures/benchmark/unlimited/avg_states_p_sec.png}
%          \caption{Average States per Second per Run}
%          \label{fig:states_per_second_unlimited}
%      \end{subfigure}
%      \hfill
%      % \begin{subfigure}[b]{0.75\linewidth}
%      %     \centering
%      %     \includegraphics[width=\linewidth]{figures/benchmark/unlimited/num_sols.png}
%      %     \caption{Number of Solutions Found}
%      %     \label{fig:sols_unlimited}
%      % \end{subfigure}
%      \caption{Lazy MAPS-RRT vs. MAPS-RRT: no $r$ bound.}
%      \label{fig:bench_unlimited}
% \end{figure}

% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.75\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figures/benchmark/limited/comp_time_success.png}
%          \caption{Total Computation Time}
%          \label{fig:compTime_limited}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.75\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figures/benchmark/limited/seg_times.png}
%          \caption{Time spent segmentating nodes}
%          \label{fig:seg_time_limited}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.75\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figures/benchmark/limited/avg_states_p_sec.png}
%          \caption{Average States per Second per Run}
%          \label{fig:states_per_second_limited}
%      \end{subfigure}
%      \hfill
%      % \begin{subfigure}[b]{0.75\linewidth}
%      %     \centering
%      %     \includegraphics[width=\linewidth]{figures/benchmark/limited/num_sols.png}
%      %     \caption{Number of Solutions Found}
%      %     \label{fig:sols_limited}
%      % \end{subfigure}
%      \caption{Lazy MAPS-RRT vs. MAPS-RRT: $r=1$ bound.}
%      \label{fig:bench_limited}
% \end{figure}

The first benchmark asks how each planner performs when we do not bound $r$. Both planners found a solution on all $1000$ runs. The results are depicted in Fig.~\ref{fig:bench_unlimited}. This scenario makes planning the top priority while explainability of the solution is a second priority. Thus, Lazy MAPS-RRT benefits from finding a solution, and then segmenting it only once. This results in Lazy MAPS-RRT planning slightly faster, generate more states per second, while also spending less time calculating segmentations. It is clear that Lazy MAPS-$\plannerX$ is more desirable than MAPS-$\plannerX$ when explainability is not the first priority. 

The second benchmark asks how each planner performs when the system needs to plan for explainability. We planned in the same space as the first benchmark, for the same amount of time, with the same planning time, and the same number of runs. However, this benchmark limited the explanation scheme to a single-segment. MAPS-RRT found $905$ solutions while Lazy MAPS-RRT only found $72$. The results are shown Figure~\ref{fig:bench_limited}. It is clear that since Lazy MAPS-$\plannerX$ only segments possible solutions, the graph $G$ fails to grow in directions with satisfiable explanations, making it extremely difficult for Lazy MAPS-$\plannerX$ to generate solutions when the optimal explanation scheme conflicts with intuitive trajectories. This scenario calls for the complete MAPS-$\plannerX$ framework, as it is capable of matching desirable system behavior with an optimal explanation scheme.  

% \begin{center}
%  \begin{tabular}{||c | c c c||} 
 
% \end{tabular}
% \end{center}

% \begin{table*}[t]
%   \centering
%   \begin{tabular}{|| c | c c c c ||}
%     \hline
%         & Solutions Found & Total Computation Time Successful Trials & Segmentation Times & Average States per Second\\ [0.5ex] 
%     \hline
%     Lazy MAPS-RRT & $1000$ & $3 \pm 2$ & $0.12 \pm 0.09$ & $1625 \pm 94$ \\ 
%     \hline
%     MAPS-RRT & $1000$ & $4 \pm 3$ & $0.8 \pm 0.5$ & $1317 \pm 75$ \\
%     \hline
%   \end{tabular}
%   \caption{Benchmark Results with no $r$ bound}
%   \label{tab:table_benchmark_unlimited}
% \end{table*}

% \begin{table*}[t]
%   \centering
%   \begin{tabular}{|| c | c c c c ||}
%     \hline
%         & Solutions Found & Total Computation Time Successful Trials & Segmentation Times & Average States per Second\\ [0.5ex] 
%     \hline
%     Lazy MAPS-RRT & $72$ & $12 \pm 9$ & $2 \pm 1$ & $1156 \pm 77$ \\ 
%     \hline
%     MAPS-RRT & $905$ & $9 \pm 6$ & $4 \pm 3$ & $887 \pm 99$ \\
%     \hline
%   \end{tabular}
%   \caption{Benchmark Results with $r=1$ bound}
%   \label{tab:table_benchmark_limited}
% \end{table*}






\subsection{Optimal MAPS Planning}
We also present examples on how our framework can be used to optimize over different objectives. First, we show MAPS-\textit{Stable Sparse RRT (SST)} \cite{li2016asymptotically}. SST is an asymptotically near-optimal motion planner for systems with kinodynamical constraints. Our MAPS variant of SST inherits these properties with the added capability of returning a satisfiable explanation scheme. Next, we append MAPS-SST to an existing meta-algorithm known as \textit{Asymptotically Optimal-$\plannerX$ (AO-$\plannerX$)} \cite{7588078}. AO-$\plannerX$ allows motion planning algorithms to optimize over any cost function by planning in the compound state-cost space. Since the cost function of MAPS-$\plannerX$ lives in $\mathbb{N}$, AO-MAPS-$\plannerX$ can be used to optimize over the number of segmentations required to explain the solution. 



\subsubsection{MAPS-SST}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsSST/example1_2ndOrderKin/seg1_crop.png}
         \caption{Time Period $[0, 20.3] s$}
         \label{fig:ex1Seg1SST}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/mapsSST/example1_2ndOrderKin/seg2_crop.png}
         \caption{Time Period $[20.3, 36.1] s$}
         \label{fig:ex1Seg2SST}
     \end{subfigure}
     \caption{Solution via MAPS-SST in open space.}
     \label{fig:ex1CarSST}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{figures/mapsSST/example2_2ndOrderUnicycle/fullPlanOneSeg_crop.png}
    \caption{MAPS-SST returns the optimal explanation scheme.}
    \label{fig:ex2_OneSegmentSST}
\end{figure}

Fig.~\ref{fig:ex1CarSST} shows the explanation scheme returned by MAPS-SST. Notice how the agents are more efficient in traveling to goal than in Fig.~\ref{fig:explanationEx1}. MAPS-SST can return near-optimal trajectories with satisfiable explanation schemes. If the user desired the plan to be explained in a single segment, MAPS-SST uses our cost function to return a near-optimal trajectory with an optimal explanation scheme. Fig.~\ref{fig:ex2_OneSegment} was a solution found by MAPS-SST while Fig.~\ref{fig:ex2_OneSegment} was a solution found by MAPS-EST. Despite both queries following the same dynamical constraints, the trajectories in Fig.~\ref{fig:ex2_OneSegment} more directly approach their goal region. 

\subsubsection{AO-MAPS-SST}
\jk{having some implementation issues with saving the plans for this planner. Working on fixing them now.}
